Meta-Learning Hypothesis Spaces for Sequential Decision-making

Obtaining reliable, adaptive confidence sets for prediction functions (hypotheses) is a central challenge in sequential decision-making tasks, such as bandits and model-based reinforcement learning. These confidence sets typically rely on prior assumptions on the hypothesis space, e.g., the known kernel of a Reproducing Kernel Hilbert Space (RKHS). Hand-designing such kernels is error prone, and misspecification may lead to poor or unsafe performance. In this work, we propose to meta-learn a kernel from offline data (Meta-KeL). For the case where the unknown kernel is a combination of known base kernels, we develop an estimator based on structured sparsity. Under mild conditions, we guarantee that our estimated RKHS yields valid confidence sets that, with increasing amounts of offline data, become as tight as those given the true unknown kernel. We demonstrate our approach on the kernelized bandit problem (a.k.a.~Bayesian optimization), where we establish regret bounds competitive with those given the true kernel. We also empirically evaluate the effectiveness of our approach on a Bayesian optimization task.

==> old_stuff/0_warmup.tex <==
\section{Warm-up: Multi Kernel Learning}\label{sec:warmup}

\subsection{Model} Consider an unknown function $f \in \gH_k$. The kernel function $k$ is mercer and resides in the Hyper-RKHS $\gH_{\underline{k}}$ as defined by \citet{ong2005learning}. The Hyperkernel $\underline{k}$ is known. We observe noisy values of the function via $y_i = f(x_i) + \epsilon_i$ where $\epsilon_i$ are independent and sub-gaussian. We further assume that the input domain is a compact and convex subspace of a euclidean space.
\comment{\small Assumption on noise can be relaxed to $(\epsilon_i)_i$ are a martingale seq. of sub-gaussian RVs.}
\subsection{Finite-Dimensional Mercer Hyper-Kernel}
We first define a Hyper-Mercer kernel, based on definition of a Hyper-RKHS from \citet{ong2005learning}. 
\later{\begin{definition}[Mercer Hyper-Kernel]
\end{definition}}

Subsequently, we drive the Mercer theorem for the Hyper-RKHS.
\later{\begin{theorem}[Mercer Decomposition of a Hyper-RKHS]
\end{theorem}}

\subsection{Kernel Learning} In the $p$-dimensional setting, members of $\gH_{\underline{k}}$ are of the form
\[k(\hx) = \sum_{i=1}^p \beta_i k_i(\hx)\]
where each $k_i(\hx)$ is Mercer and is equal to $\underline{k}(\hx, \hx_i)$ for some $\hx_i \in \gX$ and $0 \leq \beta_i$ for $1\leq i \leq p$. 
Consider the hyper-KRR problem,
\begin{equation}
    \min_{\substack{k \in \gH_{\underline{k}}\\f \in \gH_{k}}} \gL_{\mathrm{LSE}}(f, D_n) + \norm{f}^2_k + \norm{k}^2_{\underline{k}}
\end{equation}
We can show that for a $p$-dimensional hyper-kernel this problem can be reduced to
\begin{equation}\label{eq:opt_beta}
\begin{split}
            \min_{\beta}\,&\gL_{\mathrm{LSE}}(f, D_n) + \sum_{i=1}^p\frac{\norm{f}^2_{k_i}}{\beta_i}+ \norm{\vbeta}^2\\
        &\text{s.t.} \quad k = \sum_{i=1}^p \beta_i k_i, \,\, \vbeta > 0,\,\,f \in \gH_k
\end{split}
\end{equation}
Let $\hat k \in \hrkhs$ be the learned kernel, assume that it can be decomposed as 
\[k(\hx) = \sum_{i=1}^p \hat\beta_i k_i(\hx)\]
with $\hat \beta_i > 0$. Then,
\begin{prop} \label{prop:rkhs_subset}
$\gH_k \subseteq \gH_{\hat k}$.
\end{prop}
The proof is presented in the Appendix \ref{app:proofs1}. 
\begin{remark}
An RKHS $(\gH_k, k)$ is a vector space $\gH_k$ equipped with a kernel norm $\norm{\cdot}_{k}$. We only claim that function space $\gH_k$ is contained in $\gH_{\hat k}$.  The two RKHS particularly have \emph{different} kernel norms, i.e. for any $f \in \gH_k$, $\norm{f}_k \neq \norm{f}_{\hat k}$.
\end{remark}

Now in order to give a regret bound for the learner which uses $\hat k$ as its kernel function, we need to know $\norm{f}_{\hat k}$. Ideally, one would like to argue that
\[
\norm{f}_{\hat k} \leq \norm{f}_{k} \leq B.
\]
However, I don't think this would be possible, since the above property is equivalent of showing
\[
\norm{\vbeta} \leq \norm{\hat\vbeta},
\]
which would be counter intuitive given Equation \ref{eq:opt_beta}. Luckily, any other upper bound on $\norm{f}_{\hat k}$ works equally well for us. In fact, to prove a sublinear regret bound, it suffices to show:
\later{
\begin{theorem}[Upper Bound for $\vert\vert f\vert\vert_{\hat k}$]\label{thm:norm_bound}
\[
\vert\vert f\vert\vert_{\hat k} \leq  \vert\vert f\vert\vert_{k} + \Delta(n),\quad \text{w.h.p.}
\]
\end{theorem}
}
The main challenge of this setting lies in proving \cref{thm:norm_bound}. Let $\norm{f}_{k} \leq B$, then showing the following will prove the theorem,
\[
\sum_i \Big(\frac{\beta_i - \hat\beta_i}{\hat \beta_i}\Big)^2 \leq \Delta^2(n)
\]
Recall the optimization problem,
\begin{equation*}
\begin{split}
            \min_{\beta}\,&\gL_{\mathrm{LSE}}(f, D_n) + \sum_{i=1}^p\frac{\norm{f}^2_{k_i}}{\beta_i}+ \norm{\vbeta}^2\\
        &\text{s.t.} \quad k = \sum_{i=1}^p \beta_i k_i, \,\, \vbeta > 0,\,\,f \in \gH_k
\end{split}
\end{equation*}
\section{Proofs} \label{app:proofs1}
\subsection{Proofs from Section \ref{sec:warmup}}
\begin{proof}[\textbf{Proof of Proposition \ref{prop:rkhs_subset}}]
We first show that the two Hilbert spaces adopt the same orthonormal basis. Then we establish that for any $f \in \gH_k$, 
\[
\norm{f}_{\hat k} \leq \infty.
\]
The proposition follows by definition of an RKHS.
\later{\textbf{Step 1: Shared Basis}}
\paragraph{Step 2: Bounded Norm} For $f \in \gH_k$, there exists $(\alpha_r)_{r \geq 1}$ and $(\vx_r)_{r \geq 1}$ such that $f(x) = \sum_{r \geq 1}\alpha_r k(x, x_r)$. Plugging in the Decomposition of $k$ we have 
\begin{equation}
\begin{split}
    f(\vx) & = \sum_{r \geq 1} \alpha_r \sum_{i \leq p} \beta_i k_i(\vx_r, \vx)\\
    & =  \sum_{r \geq 1} \alpha_r \sum_{i \leq p} \beta_i \sum_{s \geq 1} \lambda_{i,s} \phi_{i,s}(\vx_r)\phi_{i,s}(\vx)\\
    & = \sum_{i \leq p} \beta_i \sum_{s \geq 1} \lambda_{i,s}\Big[ \sum_{r \geq 1}\alpha_r \phi_{i,s}(\vx_r)\Big]\phi_{i,s}(\vx)
\end{split}    
\end{equation}
where the second equation results by plugging in the Mercer decomposition of each $k_i(\cdot,\cdot)$, 
\[
k_i(\vx, \vx') = \sum_{s \geq 1} \lambda_{i,s}\phi_{i,s}(\vx)\phi_{i,s}(\vx').
\]
The sequence $(\phi_{i,s})_{i,s}$ is a orthonormal basis for both $\gH_k$ and $\gH_{\hat k}$. By definition, the $k$-norm of $f$ converges,
\begin{equation}\label{eq:k_norm}
    \begin{split}
        \norm{f}_{k} &= \sum_{\substack{i \leq p\\\beta_i \neq 0}} \sum_{s \geq 1} \frac{\Big( \langle f, \phi_{i,s}\rangle_{L^2} \Big)^2}{\beta_i \lambda_{i,s}}\\
        & = \sum_{\substack{i \leq p\\\beta_i \neq 0}} \sum_{s \geq 1} \frac{\Big(\lambda_{i,s} \sum_{r\geq 1}\alpha_r \phi_{i,s}(\vx_r)\beta_i \Big)^2}{\beta_i \lambda_{i,s}}\\
        & = \sum_{\substack{i \leq p\\\beta_i \neq 0}} \frac{1}{\beta_i} \sum_{s \geq 1} \lambda_{i,s} \Big( \sum_{r\geq 1}\alpha_r \phi_{i,s}(\vx_r)\beta_i \Big)^2 \leq \infty.
    \end{split}
\end{equation}
\cref{eq:k_norm} implies that for every $1\leq i \leq p$ where $\beta_i \neq 0$, the following series converges, i.e.
\begin{equation} \label{eq:k_conv}
     \sum_{s \geq 1} \lambda_{i,s} \Big( \sum_{r\geq 1}\alpha_r \phi_{i,s}(\vx_r)\beta_i \Big)^2 \leq \infty.
\end{equation}
We now proceed to show that $\norm{f}_{\hat k}$ also converges. Recall 
\[
k(\hx) = \sum_i^p \hat\beta_i k_i(\hx), \quad \hat \beta_i > 0\,\, \forall i.
\]
Then by definition of $\hat k$-norm,
\begin{equation}\label{eq:k_norm}
    \begin{split}
        \norm{f}_{\hat k} &= \sum_{i \leq p} \sum_{s \geq 1} \frac{\Big( \langle f, \phi_{i,s}\rangle_{L^2} \Big)^2}{\hat\beta_i \lambda_{i,s}}\\
        & = \sum_{i \leq p} \sum_{s \geq 1} \frac{\Big(\lambda_{i,s} \sum_{r\geq 1}\alpha_r \phi_{i,s}(\vx_r)\beta_i \Big)^2}{\hat\beta_i \lambda_{i,s}}\\
        & = \sum_{i \leq p} \frac{1}{\hat \beta_i} \sum_{s \geq 1} \lambda_{i,s} \Big( \sum_{r\geq 1}\alpha_r \phi_{i,s}(\vx_r)\beta_i \Big)^2 \\
        & = \sum_{\substack{i \leq p\\\beta_i \neq 0}} \frac{1}{\hat \beta_i} \sum_{s \geq 1} \lambda_{i,s} \Big( \sum_{r\geq 1}\alpha_r \phi_{i,s}(\vx_r)\beta_i \Big)^2\\
        & \leq \infty.
    \end{split}
\end{equation}
The last inequality follows from \cref{eq:k_conv}. 
\end{proof}
% \subsection{Bandit}
% \subsection{Regret}

==> old_stuff/early_draft.tex <==
\newpage
\section*{EARLY DRAFT}
% \section{Model}\label{sec:model_single}

% Assume we have offline data $\gD_n = \{\vx_i,y_i\}_{i\leq n}$ from one finished run of some bandit optimization task. For this data, consider the model
% \begin{equation}
%     y_i = f(\vx_i) + \varepsilon_i
% \end{equation}
% for $i \leq n$, where $\varepsilon_i$ are zero-mean i.i.d. gaussian noise with variance $\sigma^2$. We adopt a broad non-parametric characterization for the reward function $f$. Let $f \in \gH_k$ with a $B$-bounded $k$-norm, where the kernel function $k$ is unknown, however it obeys the following additive structure,
% \begin{equation}\label{eq:kernel_dec}
%     k(\vx,\vx') = \sum_{j =1}^p \eta_j k_j(\vx, \vx')
% \end{equation}
% where $k_j$ are a set of known finite-dimensional\footnote{with a potential extension to infinite-dimensional \citep{bach2008consistency}} Mercer kernels which deem \emph{plausible} for the model, and the unknown $\veta \geq 0$ can be potentially $s$-sparse. 


% Let $\vphi_j$ denote the $d_j$-dimensional feature map corresponding to the kernel $k_j$, $d = \sum_{j=1}^pd_j$, and $\vphi$ the feature map for $k$. Then $\vphi$ the feature map corresponding to $k$ is
% \[
% \vphi(\vx) = (\sqrt{\eta_1}\vphi_1^T(\vx),\cdots, \sqrt{\eta_p}\vphi_p^T(\vx))^T \in \sR^{d},
% \]
% and any function $f \in \gH_k$ may be written as
% \[
% f(\vx) =  \vphi^T(\vx) \vbeta  = \sum_{j = 1} ^ p \sqrt{\eta_j} \vphi_j^T(\vx) \vbeta^{(j)} .
% \]

% \begin{assumption}[Representability of the offline task]\label{cond:representitive}
% We assume that the function $f$ which generates $\gD_n$, is a representative member of $\gH_k$, meaning for any $\eta_j \neq 0$, we have $\vbeta^{(j)} \neq 0$. When the offline data comes from multiple tasks, then we may relax this assumption to the following. For any $\eta_j \neq 0$, there exists some task $t$, for which $\vbeta_{t,j}\neq 0$. This assumption implies that the offline tasks are diverse enough to collectively represent $\gH_k$.
% \end{assumption}

% \paragraph{Contribution} We learn a kernel $\hat k$ from this offline data, and use it to solve an online bandit problem. We show that while $\gH_{\hat k}$ does not match $\gH_k$, the learner can still attain sublinear regret, and give sufficient {\color{comment} (and in future works necessary)} conditions for sublinearity, under practical assumptions over $\gD_n$.


% To this end, we solve the following optimization problem,
% \begin{align}\label{eq:nonparam_opt}
%     \min_{\substack{\veta \geq 0,f \in \gH_k\\k = \sum_{j =1}^p \eta_j k_j}} & \frac{1}{n}\sum_{i=1}^n \left(y_i - f(\vx_i)\right)^2 
%     & + \frac{\lambda_f}{2} \norm{f}^2_k + \frac{\lambda_k}{2}\norm{\veta}_1
% \end{align}
% We may write the optimization problem (\ref{eq:nonparam_opt}) in terms of the feature maps in a parametric way,
% \begin{equation}\label{eq:generic_opt}
%     \min_{\veta\geq 0,\vbeta}  \frac{1}{n}\sum_{i=1}^n \left(y_i - \sum_{j=1}^p\sqrt{\eta_j}\vphi_j^T(\vx_i)\vbeta^{(j)}\right)^2 + \frac{\lambda_f}{2}\sum_{j=1}^p \norm{\vbeta^{(j)}}_2^2 + \frac{\lambda_k}{2}\norm{\veta}_1    
% \end{equation}
% where $\vbeta = (\vbeta^T_1, \cdots, \vbeta^T_p)^T \in \sR^d$ is the concatenation of all $\vbeta^{(j)} \in \sR^{d_j}$ so that $d=\sum_{j=1}^p d_j$. Renaming the variable $\vbeta^{(j)} \leftarrow \vbeta^{(j)}/\sqrt{\eta_j}$ gives the following equivalent problem,
% \begin{equation*}
%         \min_{\veta \geq 0,\vbeta}  \frac{1}{n}\sum_{i=1}^n \left(y_i - \sum_{j=1}^p\vphi_j^T(\vx_i)\vbeta^{(j)}\right)^2 + \frac{\lambda_f}{2}\sum_{j=1}^p \frac{\norm{\vbeta^{(j)}}_2^2}{\eta_j} + \frac{\lambda_k}{2}\norm{\veta}_1 
% \end{equation*}
% This problem is jointly convex and has an optimal solution.

% \begin{assumption}\label{cond:norm_eta}
% Without loss of generality, we can assume that $\norm{\veta}_1 \leq 1$. {\color{comment} Will explain more later.}
% \end{assumption}



%  {\color{comment} Can have an appendix section proving nice properties of this and the last optimization problem, if relevant.}


% By the \emph{$\eta$-trick} \citep{bach2004multiple}, for any two scalar variables $w$ and $v$
% \[
% \abs{w} = \min_{v\geq 0} \frac{w^2}{2v} + \frac{v}{2},
% \]
% and $\eta^* = \abs{w}$. Applying this trick with $w = \norm{\vbeta^{(j)}}_2$ and $v = \eta_j$ for all $j \leq p$ gives
% \[
%  \min_{\veta\geq 0} \frac{\lambda}{2}\sum_{j=1}^p \frac{\norm{\vbeta^{(j)}}_2^2}{\eta_j} + \frac{\lambda}{2}\norm{\veta}_1 = \lambda \sum_{j=1}^p\norm{\vbeta^{(j)}}_2.
% \]
% Under the assumption that $\lambda_k = \lambda_f$,
% for any $\vbeta$, we first optimize problem \ref{eq:generic_opt} with respect to $\veta$. Setting $\hat \veta_j = \norm{\vbeta^{(j)}}_2$, $\vy = (y_1, \cdots, y_n)$, $\mPhi = (\vphi(\vx_1), \cdots \vphi(\vx_n))^T$ gives the following equivalent optimization problem
% \begin{equation}\label{eq:glasso_opt}
%     \min_{\vbeta} \frac{1}{n}\norm{\vy -\mPhi\vbeta }_2^2 + \lambda \sum_{j=1}^p \norm{\vbeta^{(j)}}_2
% \end{equation}
% which is a kernelized variant of the Group Lasso problem \citep{yuan2006model}, with the group structure arising from the kernel decomposition given in Equation \ref{eq:kernel_dec}.

% We proceed to show that for the right choice of $\lambda$ and under a mild assumption on the offline design matrix, $\hat k$, the empirical kernel we learn via optimizing Problem \ref{eq:glasso_opt}, has desirable properties, leading to a sublinear regret for the online task. 

% \section{Properties of $\hat k$}

Let $\hat k(\vx, \vx') = \sum_{j =1}^p \hat \eta_j k_j(\vx, \vx')$, where $\hat\eta_j = \norm{\hat\vbeta^{(j)}}_2$, the solution to the group lasso problem given in \cref{eq:glasso_opt}. In future sections, we show the following
\begin{itemize}
    \item For any $f \in \gH_k$ where $\norm{f}_k \leq B$, with high probability 
    \[
    \norm{f}_{\hat k} \leq B + \epsilon(n).
    \]
        \item The set of functions spanned by $\{\hat k(\vx, \cdot), \vx\in \gX\}$ contains $\gH_k$, with high probability.
\end{itemize}
When solving the online task, the learner constructs confidence intervals using $\hat k$ as the base covariance function. The properties above allow us to produce confidence intervals with respect to the true kernel, around the unknown reward. 

We use properties of the group lasso estimator $\hat \vbeta$ to show that $\hat k$ behaves well. Next paragraph gives some insight on why the two ideas are related.

\paragraph{Estimated RKHS Norm}
Consider $f^* \in \gH_k$, with $\norm{f^*}_k^2 \leq B^2$. Then
\[f^*(\vx) = \sum_{j=1}^p \sqrt{\eta^*_j}\vphi_j^T(\vx)(\vbeta^*)^{(j)}, \quad \norm{f}_k^2 = \sum_{\substack{j \leq p\\j: \eta^*_j \neq 0}}\norm{(\vbeta^*)^{(j)}}_2^2 = \norm{\vbeta^*}_2^2.
\] 
Since $\hat \eta_j \geq 0$ and $k_i$ are Mercer, then $\hat k$ is also Mercer and we may calculate the RKHS norm with respect to $\hat k$,
\begin{equation*}
    \norm{f^*}^2_{\hat k} = \sum_{\substack{j \leq p\\ j: \hat \eta_j \neq 0}}\sum_{l=1}^{d_j} \frac{\\\left( \langle f^*, \phi_j^{(l)} \rangle_{2} \right)^2}{\hat \eta_j} = \sum_{\substack{j \leq p\\ j: \hat \eta_j \neq 0}}\sum_{l=1}^{d_j} \frac{\left( \sqrt{\eta^*_j}((\vbeta^*)^{(j)})_l\right)^2}{\hat \eta_j} = \sum_{\substack{j \leq p\\ j: \hat \eta_j \neq 0}}\frac{\eta^*_j}{\hat \eta_j}\norm{(\vbeta^*)^{(j)}}_2^2
\end{equation*}
where $\langle \cdot, \cdot \rangle_2$ denotes the inner product in the $L^2(\mathcal{X})$ space and the $\va^{(l)}$ notation shows the $l$-th element of vector $\va$. Since $\norm{\vbeta^*}_2 \leq B$, by applying Cauchy-Schwartz (multiple times) {\color{comment} [and this can be refined]}, 
\begin{equation}
    \norm{f}^2_{\hat k} \leq B^2 \sum_{\substack{j \leq p\\ j: \hat \eta_j \neq 0}} \frac{\eta^*_j}{\hat \eta_j} \leq B^2 \norm{\veta^*}_1 \max_{\substack{j\leq p\\j: \eta^*_j \neq 0,\\ \hat \eta_j \neq 0}}\frac{1}{\hat\eta_j}.
\end{equation}

Under Assumption \ref{cond:representitive}, we can give a bound on the estimated RKHS norm by showing that when $(\vbeta^*)^{(j)} \neq 0$, $\hat\vbeta^{(j)}$ is securely bounded away from zero, w.h.p. This is due to the fact that $\hat \eta_j =\norm{\hat \vbeta^{(j)}}_2$. To this end, we will give a non-asymptotic inequality which exhibits consistency, i.e. the estimated norm becomes a better approximation of $\norm{f}_k$ as $n$ grows at a $o(n^{-1/2})$ rate. 

Moreover, under Assumption \ref{cond:representitive} showing that if $(\vbeta^*)^{(j)} \neq 0$ then w.h.p. $\hat \vbeta^{(j)} \neq 0$, is equivalent to showing that the basis functions for $\gH_k$ are a subset of the basis for $\gH_{\hat k}$. Since $\hat\eta_j \neq 0$ if and only if $\hat\vbeta^{(j)} \neq 0$. 
\comment{What we aim is to show:
\[
\eta^*_j \neq 0 \xrightarrow{\mathrm{w.h.p.}} \hat\eta_j \neq 0.
\]
And the route we take is
\begin{equation*}
   \eta^*_j \neq 0 \xrightarrow{\mathrm{Cond. \ref{cond:representitive}}} (\vbeta^*)^{(j)} \neq 0  \xrightarrow{\mathrm{w.h.p}} \hat \vbeta^{(j)} \neq 0 \xleftrightarrow{\eta\mathrm{-trick}} \hat \eta_j \neq 0.
\end{equation*}
With a similar approach, we can show that if $\eta^*_j \geq c$, $\hat \eta_j \geq c - \epsilon(n)$ where $\epsilon(n) = o(n^{-1/2})$.
}
The middle step in our analysis is equivalent to showing certain variable screening properties of the group lasso estimator which lay out in the next section.

\section{Variable Screening with Kernelized Group Lasso}
For this section we follow the technique in \citet{lounici2011oracle} and occasionally use classical ideas from \citet{buhlmann2011statistics}.

We first introduce some notation. 
For any vector $\vbeta$, let $J(\vbeta) \subseteq [p]$ denote the set of active groups in $\vbeta$, where $J(\vbeta) = \{j \leq p: \vbeta^{(j)} \neq 0\}$. Moreover, for any $J \subseteq [p]$, let $\vbeta^{(j)} = (\vbeta^{(j)}\Indfunc_{j \in J})_{j\leq p} \in \sR^{d}$ denote a parameter vector which only corresponds to the groups in $J$. We will use $J^* = J(\vbeta^*)$ to denote the active groups of the true parameter. Lastly, $\bar J = [p]\setminus J$ for any $J \subseteq [p]$.

% \begin{assumption}[Normalized Base Kernels]\label{cond:normalized_kernel}
% Based kernels are normalized, i.e. for all $1\leq j \leq p$, and for all $\vx, \vx' \in \gX$, $k_j(\vx,\vx') \leq 1$.
% \end{assumption}

\begin{assumption}[Sufficient Exploration Assumption] \label{cond:RE}
There exists $\kappa = \kappa(s,\nu)$ such that
\[
\kappa \leq \min \left\{ \frac{\norm{\Phi\vb}_2}{\sqrt{n}\norm{\vb_J}_2}\,:\,\abs{J}\leq s, \,\vb\in\sR^d\setminus\{0\},\,\sum_{j \in \bar J}\lambda_j \norm{\vb_j}_2\leq \nu \sum_{j \in J}\lambda_j \norm{\vb_j}_2\right\}
\]
\end{assumption}
Consider a set of vectors in $\sR^d$, with most of their energy stored on indices in some set $J$, with $\abs{J}\leq s$. This assumption then indicates that the minimum eigenvalue of the design matrix is bounded away from zero, when restricted to the set above. In other words, for plausible parameter vectors $\vb$, there is enough exploration in the offline data.

\begin{condition}[Group Beta-min]\label{cond:betamin}
Let $\delta \in (0,1)$. For all $j \in J^*$,
\[
 \norm{(\vbeta^*)^{(j)}}_2 \geq {\color{check}c_1+c_2 \sqrt{\frac{\log 2p/\delta + \sqrt{d_\mathrm{max} \log 2p/\delta}}{n}}}.
 \]
 where $d_{\mathrm{max}} = \max_{j\leq p} d_j$ and $c_1,\,c_2$ are fixed arbitrary constants. 
\end{condition}

\begin{theorem}[Complete variable screening]\label{thm:var_screen}
Under assumption \ref{cond:RE}, if $\lambda_j$ are chosen according to lemma \ref{lem:lambda_choice}, then with probability greater than $1-\delta$
\begin{equation}
\max_{j \in J^*} \norm{\hat \vbeta^{(j)}-(\vbeta^*)^{(j)}}_2 \leq {\color{check} \frac{c}{\kappa^2} \sqrt{\frac{\log 2p/\delta + \sqrt{d_\mathrm{max} \log 2p/\delta}}{n}}},    
\end{equation}
and under condition \ref{cond:betamin},
\begin{equation}
\min_{j \in J^*} \norm{\hat\vbeta^{(j)}}_2 \geq  {\color{check} c_1 - \frac{c_3}{\kappa^2} \sqrt{\frac{\log 2p/\delta + \sqrt{d_\mathrm{max} \log 2p/\delta}}{n}}}.
\end{equation}
For some {\color{comment} calculable} constants $c_1,\, c_2, \,c_3$.
\end{theorem}

\begin{theorem} \label{thm:rkhs_screen}
Let $f \in \gH_k$. Under assumptions~\ref{cond:representitive}~to~\ref{cond:RE} and condition~\ref{cond:betamin}, and if $\lambda_j$ are chosen according to Lemma \ref{lem:lambda_choice}, with probability greater than $1-\delta$, $f \in \gH_{\hat k}$ and 
\[
\norm{f}_{\hat k} \leq B \left(1 + {\color{check}\frac{c}{\kappa} \left(\frac{\log 2p/\delta + \sqrt{d_\mathrm{max} \log 2p/\delta}}{n} \right)^{1/4}} + o(n^{-1/4})\right).
\]
\end{theorem}
Together with an RKHS confidence interval constructed for $\hat k$, Theorem \ref{thm:rkhs_screen} gives the final confidence bound needed for regret of the online task.

\subsection{Proof of Theorem \ref{thm:var_screen}}
\begin{lemma}[Right choice of $\lambda$]\label{lem:lambda_choice}
Let $A = \cup_{j\leq p} A_j$ where
\[
A_j = \left\{  \frac{1}{n} \norm{(\Phi_X^T\vvarepsilon)_j} \leq \lambda_j/2\right\}.
\]
Under assumption \ref{cond:normalized_kernel}, $\sP(A)\geq 1-\delta$ if for all $j \leq p$
\[
\lambda_j \geq \frac{2\sigma}{\sqrt{n}}\sqrt{1 + \frac{2}{n}\log (2p/\delta) + \frac{2}{n}\sqrt{d_j \log( 2p/\delta)}}
\]
\end{lemma}
\begin{lemma}[Properties of $\hat \vbeta$ conditioned on $A$]
If event $A$ happens, the $\hat \vbeta$ the group lasso estimator satisfies the following
\begin{align}
     &\frac{1}{n} \norm{\Phi_X(\hat \vbeta-\vbeta^*)}_2^2 + \sum_{j=1}^p\lambda_j \norm{\hat \vbeta^{(j)}-\vbeta^{(j)}} \leq \frac{1}{n} \norm{\Phi_X(\vbeta-\vbeta^*)}_2^2 \notag\\
     & \qquad\qquad+ 4 \sum_{j \in J(\vbeta)} \lambda_j \min\left( \norm{\vbeta^{(j)}}, \norm{\hat\vbeta^{(j)}-\vbeta^{(j)}}\right)\label{eq:basic_ineq}\\
    &\frac{1}{n} \norm{\Big(\Phi^T_X\Phi_X(\hat \vbeta-\vbeta^*)\Big)_j}  \leq \frac{3}{2} \lambda_j\label{eq:empproc_lambda}
\end{align}
where the first inequality holds  for all $\vbeta\in \sR^d$.
\end{lemma}

\section{Multi-task Setting}
% We now consider the setting where there is data available from $m$ tasks, each of sample size $n$. Let $\gD_n^{(s)} = \{\vx_{s,i}, y_{s,i} \}_{i \leq n}$ for $1\leq s\leq m$. For each task $s$ the data generating model obeys
% \[
% y_{s,i} = f_{s}(\vx_{s,i})+\varepsilon_{s,i}
% \]
% for $i \leq n$, where $f_s \in \gH_k$ with an RKHS norm bounded by $B$. The kernel $k$ is shared among all tasks and has the form
% \[
% k(\vx,\vx') = \sum_{j=1}^p\eta_j k_j(\vx,\vx')
% \]
% where $\eta_j$ are to be learned and $k_j$ are known finite-dimensional Mercer kernels. We define the corresponding feature maps similar to section \ref{sec:model_single} and so
% \[
% f_s(\vx) = \vphi^T(\vx)\vbeta_s=\sum_{j=1}^p \sqrt{\eta_j}\vphi_j^T(\vx)\vbeta_s^{(j)}
% \]
% where $\vbeta_s^{(j)}\in \sR^{d_j}$ and $\vbeta_s \in \sR^d$ with $d = \sum_{j\leq p}d_j$. 
% To learn $\veta$, we solve the following optimization problem,
% \[
% \min_{\substack{\vbeta_s, \veta\\s\leq m}} \frac{1}{m} \sum_{s=1}^m \left[ \frac{1}{n}\sum_{i=1}^n \left( y_{s,i} - \sum_{j=1}^p \sqrt{\eta_j}\vphi_j^T(\vx_{s,i})\vbeta_s^{(j)}\right)\right] + \frac{\lambda}{2} \sum_{s=1}^m\sum_{j=1}^p\norm{\vbeta_s^{(j)}}_2^2 + \frac{\lambda}{2}\norm{\veta}_1.
% \]
% Renaming the variable $\vbeta_s^{(j)} \leftarrow \vbeta_s^{(j)}/\sqrt{\eta_j}$ gives the following equivalent problem,
% \[
% \min_{\substack{\vbeta_s, \veta\\s\leq m}} \frac{1}{m} \sum_{s=1}^m \left[ \frac{1}{n}\sum_{i=1}^n \left( y_{s,i} - \sum_{j=1}^p \vphi_j^T(\vx_{s,i})\vbeta_s^{(j)}\right)\right] + \frac{\lambda}{2} \sum_{j=1}^p\frac{\sum_{s=1}^m\norm{\vbeta_s^{(j)}}_2^2}{\eta_j} + \frac{\lambda}{2}\norm{\veta}_1.
% \]
% Applying the $\eta$-trick, we get that $\hat\eta_j = \sqrt{\sum_{s\leq m} \norm{\vbeta_s^{(j)}}^2_2}$ and the optimization problem becomes
% \begin{equation}\label{eq:multi_loss_raw}
% \min_{\substack{\vbeta_s\\s\leq m}} \frac{1}{m} \sum_{s=1}^m \left[ \frac{1}{n}\sum_{i=1}^n \left( y_{s,i} - \sum_{j=1}^p \vphi_j^T(\vx_{s,i})\vbeta_s^{(j)}\right)\right] + \lambda \sum_{j=1}^p\sqrt{\sum_{s=1}^m\norm{\vbeta_s^{(j)}}_2^2}.
% \end{equation}
% We now proceed to show that Problem \ref{eq:multi_loss_raw} is also equivalent to a Group Lasso problem, defined on a different feature matrix and parameter vector.  

% \paragraph{Group Lasso Formulation of the Multi-task Setting} We let $\vy_s \in \sR^{n}$ denote the observed reward values for task $s$ and $\vy = (\vy_1^T,\cdots,\vy_m^T)^T \in \sR^{mn}$ the complete vector. Similarly we define $\vbeta = (\vbeta^T_1,\cdots,\vbeta^T_m)^T \in \sR^{md}$ the concatenated parameter vector for all tasks. 
% Finally, to show the indices belonging to the $j$-th group across all tasks, we use $\vbeta^{(j)} = (\vbeta^T_{1,j},\cdots,\vbeta^T_{m,j})^T \in \sR^{md_j}$. Note that the second term in the loss function \ref{eq:multi_loss_raw} can be written as
% \[
% \sum_{j=1}^p \sqrt{\sum_{s=1}^m \norm{\vbeta_s^{(j)}}_2^2} = \sum_{j=1}^p \norm{\vbeta^{(j)}}_2.
% \]
% It remains to define the cross-task feature matrix $\mPhi \in \sR^{mn\times md}$ which is a block-diagonal matrix, where each block $s$ corresponds to $\mPhi_s^T = (\vphi(\vx_{s,1}), \cdots, \vphi(\vx_{s,n}))$, $n\times d$ the feature matrix of task $s$. Using the multi-task notation we get,
% \begin{equation}\label{eq:glasso_opt_multi}
% \min_{\vbeta^{(j)}} \frac{1}{mn} \norm{\vy-\mPhi\vbeta}_2^2 + \lambda \sum_{j=1}^p \norm{\vbeta^{(j)}}_2
% \end{equation}

% Comparing to problem \ref{eq:glasso_opt}, we can see that the group structure is the same, and induced by the kernel definition. The size of each group is multiplied by $m$ the number of tasks, as indices of $\vbeta_s$ corresponding to a group $j$ across all tasks are grouped together. As expected, the size of the dataset has also increased from $n$ to $mn$. In this setting the estimated kernel $\hat k(\vx, \vx') = \sum_{j =1}^p \hat \eta_j k_j(\vx, \vx')$, where $\hat\eta_j = \norm{\hat\vbeta^{(j)}}_2$, and $\hat\vbeta$ is the solution to the multi-task group lasso problem (\cref{eq:glasso_opt_multi}).

% \paragraph{Multi-task Assumptions} The sufficient assumptions in the multi-task setting are in fact a relaxed version of the assumptions we required for our single-task analysis.
% \begin{assumption}[Collective Representability - relaxed version of Assumption \ref{cond:representitive}]\label{cond:representative_relaxed}
% We assume that for any $\eta_j \neq 0$, there exists some task $s$ in the meta dataset for which $\vbeta^{(j)}_s \neq 0$. This assumption implies that the offline tasks are diverse enough to collectively span $\gH_k$.
% \end{assumption}


\begin{theorem}[Complete variable screening with Meta-data]\label{thm:var_screen_multi}
If assumption \ref{cond:RE} holds for each $\mPhi_s$, and for all $1\leq j \leq p$ 
\[
\lambda_j \geq \frac{2\sigma}{\sqrt{nm}}\sqrt{1 + \frac{2}{nm}\left( \log (2p/\delta) + \sqrt{md_j \log( 2p/\delta)}\right)}
\]
then with probability greater than $1-\delta$,
\begin{equation}
\max_{j \in J^*} \norm{\hat \vbeta^{(j)}-(\vbeta^*)^{(j)}}_2 \leq {\color{check} \frac{c}{\kappa^2 \sqrt{nm}} \sqrt{\log 2p/\delta + \sqrt{md_\mathrm{max} \log 2p/\delta}}},    
\end{equation}
and under condition \ref{cond:betamin},
\begin{equation}
\min_{j \in J^*} \norm{\hat\vbeta^{(j)}}_2 \geq  {\color{check} c_1 - \frac{c_3}{\kappa^2\sqrt{nm}} \sqrt{\log 2p/\delta + \sqrt{md_\mathrm{max} \log 2p/\delta}}}.
\end{equation}
For some {\color{comment} calculable} constants $c_1,\, c_2, \,c_3$.
\end{theorem}


\begin{theorem} \label{thm:meta_rkhs_screen}
Let $f \in \gH_k$. Assume $\vbeta^*$ satisfies condition \ref{cond:RE} and assumption \ref{cond:representative_relaxed} holds for every $\mPhi_s$, $s\leq m$ for some $\kappa$. Then under assumptions~\ref{cond:norm_eta}, ~\ref{cond:normalized_kernel}~and~\ref{cond:representative_relaxed}, with probability greater than $1-\delta$, $f \in \gH_{\hat k}$ and 
\[
\norm{f}_{\hat k} \leq B \left(1 + \frac{c}{\kappa} \left(\frac{\log 2p/\delta + \sqrt{md_\mathrm{max} \log 2p/\delta}}{nm} \right)^{1/4} + o((nm)^{-1/4})\right).
\]
\end{theorem}




==> old_stuff/old_experiments.tex <==
\section{Experiments}

\paragraph{MetaLearning}
We use the Fourier features and construct each feature map $\vphi_j$ as follows,
\[
\vphi_j(x) = \left(\sin(jdxf_0), \cos(jdxf_0), \cdots, \sin((j+1)dxf_0),\cos((j+1)dxf_0 \right)
\]
\[
\vphi_p(x) = (\alpha_1(x-\alpha_2)^{\alpha_3}) 
\]
where $f_0$ is some base frequency. Then each frequency kernel $k_j(x,x')=\vphi_j^T(x)\vphi(x')$ covers a discrete frequency band of width $d$, $[jdf_0, (j+1)df_0]$, and the last kernel creates a polynomial which essentially determines the global optima. In this setting, the kernel sparsity translates to the signals being sparse in the frequency domain, which is often the case for natural signals, i.e. image and speech. 
% \begin{figure}
%     \centering
%     \includegraphics[width = 0.4\linewidth]{figures/exp0_p5_s2_n1000_d2.pdf}
%     \caption{Recovering the kernel and estimating the functions from 1000 noisy samples of 5 offline tasks. There are 5 total kernels, each have 2 frequencies, only 2 are active. The correct kernels are chosen by group lasso.}
%     \label{fig:recovering4}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width = 0.9\linewidth]{figures/exp0_p5_s2_n1000.pdf}
%     \caption{Recovering the kernel and estimating the functions from 1000 noisy samples of 7 offline tasks. There are 5 total kernels, each have 3 frequencies, only 2 are active. The correct kernels are chosen by group lasso.}
%     \label{fig:recovering0}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[height = 0.35\paperheight]{figures/exp0_p5_s2_n1000_d4.pdf}
%     \caption{ \label{fig:recovering1} Recovering the kernel and estimating the functions from 1000 noiseless samples of 3 offline tasks. There are 5 total kernels, each have 4 frequencies, only 2 are active. The correct kernels are chosen by group lasso.}
%     \includegraphics[height = 0.35\paperheight]{figures/exp0_p5_s3_n1000_d4.pdf}
%     \caption{ \label{fig:recovering2} Recovering the kernel and estimating the functions from 1000 noiseless samples of 3 offline tasks. There are 5 total kernels, each have 4 frequencies, only 3 are active. The correct kernels are chosen by group lasso.}
% \end{figure}
% \begin{figure}
% \centering
%     \includegraphics[height = 0.35\paperheight]{figures/exp0_p3_s2_n1000_d4.pdf}
%     \caption{\label{fig:recovering5} Recovering the kernel and estimating the functions from 1000 noiseless samples of 4 offline tasks. There are 3 total kernels, each have 4 frequencies, only 2 are active. The correct kernels are chosen by group lasso.}
%     \includegraphics[height = 0.35\paperheight]{figures/exp0_p3_s2_n100_d4.pdf}
%     \caption{\label{fig:recovering3} Recovering the kernel and estimating the functions from 100 noiseless samples of 4 offline tasks. There are 3 total kernels, each have 4 frequencies, only 2 are active. The correct kernels are chosen by group lasso.}
% \end{figure}

% \paragraph{Kernel Recovery}
% For different $\gamma = s/p$ ratios, we compare the empirical probability of kernel recovery with the theoretical one.
% From Theorem \ref{thm:var_screen_multi}
% \[
% \delta \geq 2p\exp\left\{\frac{\sqrt{md_{\mathrm{max}}} - \sqrt{md_{\mathrm{max}}+4nmC(s)}}{2} \right\}
% \]

% where $C(s)$ depends on $\kappa(s)$ the sufficient exploration constant.

% \begin{figure}
% \centering
%     \begin{minipage}{0.4\textwidth}

%     \includegraphics[width = 0.8\textwidth]{figures/exp0_violin_runs20_n1000.pdf}
%   \caption{
%     \label{fig:recovery_violin1}Distribution of number of estimated active groups $\left\vert \{\hat\eta_j \neq 0 \}\right\vert$. Regularization parameters $\lambda_j$ are picked according to Theorem \ref{thm:var_screen_multi}.}
% \end{minipage}
% \begin{minipage}{0.4\textwidth}
%     \includegraphics[width = 0.8\textwidth]{figures/exp0_violin_runs20_n1000_handlambdas.pdf}
%     \caption{
%     \label{fig:recovery_violin2}Distribution of number of estimated active groups $\left\vert \{\hat\eta_j \neq 0 \}\right\vert$. Regularization parameters $\lambda_j$ are picked by hand, but not tuned severely.}
% \end{minipage}
% \end{figure}
\begin{figure}
    \centering
    \includegraphics[width = 0.5\textwidth]{figures/Bo_samples.png}
    \caption{How Meta-BO is sampling the domain.}
\end{figure}
\begin{figure}[ht]
\centering
    \begin{minipage}[t]{0.6\textwidth}
    \centering
    \includegraphics[height = 0.7 \textwidth]{figures/oracle_PolyFreq_10run_regret_5p_3d_2s_1000n_20m_500T.pdf}
    \caption{\label{fig:regret_curves_oracle} Simple Regret and the Cumulative Regret for the Oracle, i.e. true kernel $\tk$ is known by the BO algorithm.}
\end{minipage}
\begin{minipage}[t]{0.3\textwidth}
    \centering
    \includegraphics[height = 1.2\textwidth]{figures/task_size.png}
    \caption{\label{fig:exp_offline_tasknum} Effect of increasing the number of tasks from $m=2$ to $m=20$ on $R(500)$. Each task is of size $n = 500$. }
\end{minipage}
\end{figure}
\begin{figure}[ht]
\centering
    \begin{minipage}{0.45\textwidth}
    \centering
    \includegraphics[width = 0.9\textwidth]{figures/sparse_PolyFreq_10run_regret_5p_3d_2s_500n_20m_500T.pdf}
  \caption{
    \label{fig:regret_curves_sparse}  Simple Regret and the Cumulative Regret for the \ourmethod. Here the true kernel $\tk$ is not known by the BO algorithm, and the candidate kernels are selected via meta-learning, using $m=10$ tasks of length $n=1000$.}
\end{minipage}
\begin{minipage}{0.45\textwidth}
\centering
    \includegraphics[width = 0.9\textwidth]{figures/full_PolyFreq_10run_regret_5p_3d_2s_500n_20m_500T.pdf}
    \caption{
    \label{fig:regret_cruves_sparse}  Simple Regret and the Cumulative Regret for the Complex Model. Here the true kernel $\tk$ is not known by the BO algorithm, and all candidate kernels are set to active, i.e. $\etahat_j = 1$ for all $j \leq p$.}
\end{minipage}
\end{figure}




==> old_stuff/outline.tex <==
\onecolumn
\section{Working Outline}
\begin{enumerate}
    \item Intro
    \begin{itemize}
        \item Open with BO. With don't know the objective. We need to make some hypothesis.
        \item If the hypothesis space doesn't match the true space, we can not find the optima. 
        \item It is \textbf{impossible} to guarantee convergence of the BO if the hypothesis space does not contain the true space.
        \item We often don't know what is the true function space. General solution? Pick one that is certainly much more complex.
        \item When the function space is unknown, but we have some knowledge about the structure (RKHS with additive kernel), we aim to find a \emph{tight} hypothesis space via meta-learning.
        \begin{figure}[ht]
            \centering
            \subfigure[]{\includegraphics[width = 0.25\textwidth]{figures/wrong_rkhs.pdf}}
            \subfigure[]{\includegraphics[width = 0.25\textwidth]{figures/large_rkhs.pdf}}
            \subfigure[]{\includegraphics[width = 0.25\textwidth]{figures/tight_rkhs.pdf}}
            \caption{(a) Wrong Hypothesis Space (b) Complex Hypothesis Space (c) Meta-Learned Hypothesis Space}
            \label{fig:hypothesis}
        \end{figure}
        \item Related Work {\color{comment} Here or in the very end before conclusion?}
        \begin{itemize}
            \item sparse bandits
            \item MKL
            \item Meta learning and bandits
            \item BO with complex kernels/ Neural bandits
        \end{itemize}
        \item Contributions
        \begin{itemize}
        \item We present a meta-learning approach which any kernelized BO method can be plugged into.
            \item We work in a setting when the function space is a RKHS with unknown kernel, but the kernel has a certain structure.
            \item The meta-learned RKHS is  \emph{non-complex} and with high probability contains the true RKHS.  
            \item We further bound the true unknown RKHS norm with the RKHS norm of the meta-learned space.
            \item For the BO problem: We give valid confidence intervals for the unknown objective, without knowledge of the true RKHS.
            \item For any BO method that guarantees convergence ($\vert f(x^*)-f(x_t)\vert  \leq \epsilon$) with knowledge of the RKHS, we guarantee convergence even when the RKHS is unknown, in presence of enough meta-data (poly rate with $\epsilon^{-1}$).
        \end{itemize}
    \end{itemize}
    \item Problem Setting
    \begin{itemize}
        \item No background section. We'll give rkhs and group lasso overviews in the appendix.
        \item Assumption on how the meta-data is generated. We have been given the offline data.
        \item The representability assumption (but as part of the model, plus footnote)
        \item how the BO task relates to the offline task 
        \item assumption on the BO setup
    \end{itemize}
    
    \item Meta-Learning the function space
    
    %%%
    


    %%%
    \begin{itemize}
\item subsection 0: overview
\begin{itemize}
        \item we meta-learn $\etahat, \khat$.
    \item we can then plug this $\khat$ into any GP-BO method.
\end{itemize}
        \item subsection 1: the meta problem
        \begin{itemize}
    \item how do we learn it? the meta-optimization problem in RKHS notation
    \item we proceed to show that this is in fact very easy to solve, it is similar to a group lasso with a special group structure and will result in a sparse $\etahat$.
    \item for background on group lasso see appendix \ref{app:glasso}
    \item steps towards lasso and eta trick
    \item final format before complete group lasso
    \item define the multi task phi, beta, and any notation required for group lasso
    \item derive the group lasso
    \item let $\betahat$ and $\etahat$ be the solutions. by the $\eta$-trick, we have $\etahat_j = \norm{\betahat^{(j)}}_2$.
    \item favorable properties of the group lasso optimization problem
        \end{itemize}
  \item subsection 2: properties of $\khat$ the solution of the meta problem
\begin{itemize}
    \item sufficient exploration assumption
    \item Beta-min condition
    \item \textbf{First main theorem}:
    $\gH_k \subset \gH_{\hat k}$ and $\norm{f}_{\hat k} \leq \norm{f}_{k } + \epsilon(n)$
    \item discuss what this theorem means.
    \item This is a tough as variable screening for the group lasso problem. This result matches the optimal group lasso rate.
    \item Comparison with using $\vetahat = 1$.
    \item Consistency: more meta data means better approximation. The rate is poly.
    \item proof sketch: how this is done via group lasso variable screening
\end{itemize}
    \item conclude that meta-learning is done.
    \end{itemize}
    \item Bayesian Optimization with Meta-Learned Hypothesis [outdated]
    \begin{itemize}
        \item we take the meta-learned $\hat k$ and plug it into some BO algorithm.
        \item as an example, the Meta-GP-UCB acquisition function.
        \item \textbf{Second main theorem}: Confidence Interval for $f_{\mathrm{BO}}$: Denote the history by $H_t$. No assumption other than the fact that $x_t$ only depends on $H_{t-1}$. The true $f_{\mathrm{BO}}$ is contained between the Meta-UCB and Meta-LCB with high probability.
        \item Corollary: Meta-GP-UCB Regret Bound
        \item Corollary: this is better than the lowerbounds for using the full kernel $\vetahat=1$.
    \end{itemize}
    \item Experiments
    \begin{enumerate}
        \item Comparison of the Oracle, the Meta-GP-UCB and the full kernel GP-UCB. How Meta-GP-UCB converges the oracle with more offline data.
        \item Regret Curves for the three methods, + misspecified setting, + underspecified setting.
        \item True RKHS is always contained in the meta-learned one.
        \item Experiment on real data
    \end{enumerate}
    \item Conclusion
\end{enumerate}


Questions

- Is it clear from the intro what's the complete procedure?
- What does he think about the way the assumptions are presented?
- Clarity of theorem 3.3
- properties of structures sparsity?
- we have sublinear regret for meta-kel on vaccine, should we include it?
- drop the oracle notation?
- Explain related work. Should I drop something?
- We have some space, should I bring back the figures? what should I do?
